Key Feature Replacement of In-Distribution Samples for Out-of-Distribution Detection

Out-of-distribution (OOD) detection can be used in deep learning-based applications to reject outlier samples from being unreliably classified by deep neural networks. Learning to classify between OOD and in-distribution samples is difficult because data comprising the former is extremely diverse. It has been observed that an auxiliary OOD dataset is most effective in training a "rejection" network when its samples are semantically similar to in-distribution images. We first deduce that OOD images are perceived by a deep neural network to be semantically similar to in-distribution samples when they share a common background, as deep networks are observed to incorrectly classify such images with high confidence. We then propose a simple yet effective Key In-distribution feature Replacement BY inpainting (KIRBY) procedure that constructs a surrogate OOD dataset by replacing class-discriminative features of in-distribution samples with marginal background features. The procedure can be implemented using off-the-shelf vision algorithms, where each step within the algorithm is shown to make the surrogate data increasingly similar to in-distribution data. Design choices in each step are studied extensively, and an exhaustive comparison with state-of-the-art algorithms demonstrates KIRBY's competitiveness on various benchmarks.

==> tables/ablation_psi.tex <==
\begin{table*}[]
\begin{adjustbox}{width=14.0cm,center}
\begin{tabular}{c|ccc|ccc|ccc} \toprule
 \multirow{2}{*}{$\hat{\Psi}$}
 & \multicolumn{3}{c}{WideResNet} & \multicolumn{3}{c}{ResNet} & \multicolumn{3}{c}{DenseNet} \\ 
 \cline{2-10}
 & CIFAR-10 & CIFAR-100 & STL-10 & CIFAR-10 & CIFAR-100 & STL-10 & CIFAR-10 & CIFAR-100 & STL-10 \\ \midrule
KIRBY-M & 90.54 & 77.21 & 76.92 & 90.97 & 73.02 & 75.36 & 92.49 & 78.60 & 77.76 \\
KIRBY-B & \textbf{97.82} & \textbf{93.11} & 88.79 & \textbf{97.51} & \textbf{90.44} & 82.30 & 96.54 & 92.99 & 88.59 \\
KIRBY-R & 97.03 & 92.31 & \textbf{89.50} & 96.94 & 88.32 & \textbf{84.74} & \textbf{97.03} & \textbf{93.57} & \textbf{91.25} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Ablation study on $\hat{\Psi}$ assessing binary (B) vs. $K+1$ classification with MSP over ID classes (M) and reject class (R). Entries are the area under the receiver operating characteristic curve (AUROC) with column ID sets, averaged over all OOD sets described in the experiment section.
% We report average AUROC over six OOD datasets mentioned in Section~\ref{sec:setup}.
}
\label{tab:ablation_psi}
\end{table*}

==> tables/binary_classifier.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
% \begin{adjustbox}{width=8.3cm,center}
\begin{center}
% \begin{small}
    \begin{tabular}{c|c|cccccc} \toprule
     &  & \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{c}{\textbf{STL-10}} 
     \\
    Method & Block \# & FRP $\downarrow$ & AUROC $\uparrow$ & FPR $\downarrow$ & AUROC $\uparrow$ & FPR $\downarrow$ & AUROC $\uparrow$ \\ \midrule
    \multirow{3}{*}{\textbf{Grad-CAM}} 
     & 1 & 17.67 & 96.33 & 37.38 & 90.90 & 52.30 & 87.45 \\
     & 2 & 18.36 & 95.96 & 37.91 & 91.09 & 49.37 & 88.34 \\
     & 3 & 14.27 & 96.96 & \textbf{33.39} & \textbf{92.41} & \underline{44.92} & 89.10 \\ \bottomrule
    \end{tabular}
    % \end{small}
\end{center}
% \end{adjustbox}
\label{tab:ablation_cam}
\caption{Influence of CAM variants on downstream out-of-distribution performance. Block \# indicates the hidden block in WRN-40-2 at which CAM features were extracted.}
\end{table}

==> tables/cifar100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{adjustbox}{width=11cm,center}
\begin{tabular}{c|c|cccccccccccc}
\multirow{4}{*}{\textbf{IND}} & \multirow{4}{*}{\textbf{Method}} & \multicolumn{10}{c}{\textbf{OOD Datasets}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}} \\
 &  & \multicolumn{2}{c}{\textbf{SVHN}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{LSUN-crop}} & \multicolumn{2}{c}{\textbf{LSUN-resize}} & \multicolumn{2}{c}{\textbf{Place365}} & \multicolumn{2}{c}{} \\
 &  & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC \\ 
 &  & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ \\ \hline
\multirow{3}{*}{Cifar10} 
 & Ours-GradCam &  11.01 &  97.88 &  39.39 &  90.41 &  4.43 &  99.03 &  24.61 &  95.27 & 24.61 &  95.27 &  22.44 &  95.08 \\
 & Ours-GradCampp & \textbf{10.37} & \textbf{97.96} & 38.97 & 90.38 & \textbf{4.26} & \textbf{99.05} & 24.37 & 95.27 & 24.37 & 95.27  & 22.12 & 95.09 \\
 & Ours-LayerCam & 10.67 & 97.91 & \textbf{38.85} & \textbf{90.44} & 4.33 & \textbf{99.05} & \textbf{24.16} & \textbf{95.31} & \textbf{24.16} & \textbf{95.31}  & \textbf{22.11} & \textbf{95.11} \\ \hline

\multirow{3}{*}{Cifar100} 
 & Ours-GradCam &  13.09 &  97.61 &  63.11 &  83.66 &  21.74 & 96.21 & 57.21 & 87.64 & 57.21 & 87.64 & 46.50 &  88.44 \\
 & Ours-GradCampp & 12.92 & 97.61 & 62.31 & 83.81 & \textbf{20.56} & \textbf{96.38} & \textbf{56.28} & \textbf{87.80} & \textbf{56.28} & \textbf{87.80}  & 45.73 & 88.60 \\
 & Ours-LayerCam & \textbf{12.66} & \textbf{97.66} & \textbf{62.12} & \textbf{84.02} & 21.02 & 96.31 & 57.93 & 87.24 & 57.93 & 87.24 & \textbf{46.05} &  \textbf{88.60} \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Comparison result for various weakly supervised localization methods.}
\label{tab:torn_ablation_ws}
\end{table}

==> tables/imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{adjustbox}{width=11cm,center}
\begin{tabular}{c|c|cccccccccc}
\multirow{4}{*}{\textbf{IND}} & \multirow{4}{*}{\textbf{Method}} & \multicolumn{8}{c}{\textbf{OOD Datasets}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}} \\
 &  & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Place365}} & \multicolumn{2}{c}{\textbf{Textures}} &  \multicolumn{2}{c}{} \\
 &  & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC \\ 
 &  & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ \\ \hline
\multirow{6}{*}{ImageNet} 
 & MSP &  54.99 &  87.74 &  70.83 & 80.86 & 73.99 & 79.76 & 68.00 & 79.61 & 66.95 & 81.99  \\
 & ODIN & 47.66 & 89.66 & 60.15 & 84.59 & 67.89 & 81.78 & 50.23 & 85.62 & 56.48 & 85.41   \\
 & Energy & 55.72 & 89.95 & 59.26 & 85.89 & 64.92 & 82.86 & 53.72 & 85.99 & 58.41 & 86.17 \\
 & ReAct & 45.69 & 91.88 & 56.80 & 87.35 & 62.23 & 85.24 & 57.82 & 86.91 & 55.63  & 87.85  \\
 & Mahalanobis & 97.00 & 52.65 & 98.50 & 42.41 & 98.40 & 41.79 & 55.80 & 85.01 & 87.43 & 55.47 \\ \cline{2-12}
 & Ours & \textbf{10.67} & \textbf{97.91} & \underline{38.85} & \underline{90.44} & \textbf{4.33} & \textbf{99.05} & \textbf{24.16} & \textbf{95.31} & \textbf{24.16} & \textbf{95.31} \\ \hline

 
\end{tabular}
\end{adjustbox}
\caption{Comparison with competitive post hoc OOD detection methods.}
\label{tab:imagenet_result}
\end{table}

==> tables/ind_accuracy.tex <==
\begin{table}[]
\caption{Test dataset (IND) accuracies. All values are percentages.
{\color{red}What's this for?}
}
\begin{adjustbox}{width=11cm,center}
\begin{tabular}{c|ccc|ccc|ccc} \toprule
 & \multicolumn{3}{c}{\textbf{WideResNet}} & \multicolumn{3}{c}{\textbf{ResNet}} & \multicolumn{3}{c}{\textbf{DenseNet}} \\ 
 IND & CIFAR-10 & CIFAR-100 & STL-10 & CIFAR-10 & CIFAR-100 & STL-10 & CIFAR-10 & CIFAR-100 & STL-10  \\ \hline
Accuracy (\%) & 94.84 & 75.96 & 81.25 & 93.67 & 78.34 & 80.27 & 95.40 & 77.28 & 86.15  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:ind_acc}
\end{table}

==> tables/layers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{adjustbox}{width=11cm,center}
\begin{tabular}{c|c|cccccccccccc}
\multirow{4}{*}{\textbf{IND}} & \multirow{4}{*}{\textbf{Layer}} & \multicolumn{10}{c}{\textbf{OOD Datasets}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}} \\
 &  & \multicolumn{2}{c}{\textbf{SVHN}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{LSUN-crop}} & \multicolumn{2}{c}{\textbf{LSUN-resize}} & \multicolumn{2}{c}{\textbf{Place365}} & \multicolumn{2}{c}{} \\
 &  & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC \\ 
 &  & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ \\ \hline
\multirow{3}{*}{Cifar10} 
 & Layer1 & 51.16 & 88.01 & 68.62 & 79.04 & 12.17 & 97.82 & 68.94 & 86.25 & 68.94 & 86.25  & 53.4 & 87.30 \\
 & Layer2 &  42.07 &  88.76 & 54.31 & 83.27 & 3.70 & 99.11 & 39.24 & 91.77 & 39.24 & 91.77 & 37.53 & 90.39 \\
 & Layer3 & \textbf{10.67} & \textbf{97.91} & \textbf{38.85} & \textbf{90.44} & \textbf{4.33} & \textbf{99.05} & \textbf{24.16} & \textbf{95.31} & \textbf{24.16} & \textbf{95.31}  & \textbf{22.11} & \textbf{95.11} \\ \hline

\multirow{3}{*}{Cifar100} 
 & Layer1 &  90.54 &  56.28 & 93.64 & 53.61 & 94.50 & 62.14 & 77.28 & 75.55 & 77.28 & 75.56 & 89.57 &  60.98 \\
 & Layer2 & 77.59 & 66.59 & 87.59 & 61.16 & 62.80 & 81.95 & 94.05 & 61.25 & 94.05 & 61.25 & 81.81  & 65.71 \\
 & Layer3 & \textbf{12.66} & \textbf{97.66} & \textbf{62.12} & \textbf{84.02} & \textbf{21.02} & \textbf{96.31} & \textbf{57.93} & \textbf{87.24} & \textbf{57.93} & \textbf{87.24} & \textbf{46.05} &  \textbf{88.60} \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Ablation study of applying the proposed method on different layers.}
\label{tab:torn_ablation_layers}
\end{table}
